Does Notation Matter? MusicXML Tokenisation for Symbolic Music Generation and Understanding

Symbolic music representations encode musical content at varying levels of completeness, from performance-oriented formats such as MIDI to fully notated scores such as MusicXML. Yet the impact of this representational richness on deep learning models remains poorly understood. While tokenisation has been extensively studied for MIDI, score-based formats have received considerably less attention, and MusicXML in particular remains largely unexplored despite being the de-facto standard for score interchange. In this paper, we introduce the first general-purpose tokenisation framework for MusicXML, and conduct a systematic empirical study to determine whether notational richness confers a measurable advantage for deep learning on symbolic music. We train 26 autoregressive and masked language models, comparing MusicXML tokenisation against MIDI and ABC-based representations, probing the effect of different tokenisation strategies within MusicXML, and testing whether music-grammar-aware tokenisation outperforms treating scores as plain text. We evaluate music understanding tasks using linear probing across composer classification, difficulty estimation, and accompaniment suggestion, and generative tasks using objective statistical metrics and a human pairwise preference study. Our results show that MusicXML-tokenised models outperform MIDI and text-based counterparts on understanding and generative tasks.

==> tables/gpt_automatic.tex <==
add a line for every tokenizer for the 5k BPE:
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llccccc}
\toprule
\textbf{Tokenizer} & \textbf{BPE} & \textbf{PR} & \textbf{SC} & \textbf{GC} & \textbf{JS} $\uparrow$ \\
\midrule
\multirow{2}{*}{\libraryName\--MF} & 10k & 28.6 & 0.98 & 0.90 & \textbf{86.7} \\
                            & --  & 21.2 & 0.98 & 0.85 & 83.9 \\
\addlinespace
\multirow{2}{*}{\libraryName\--PF} & 10k & 21.0 & 0.96 & 0.79 & 85.0 \\
                            & --  &  9.3 & 0.99 & 0.77 & 67.4 \\
\midrule
\multirow{2}{*}{MIDItok--REMI} & 10k & 41.6 & 0.94 & 0.96 & 81.7 \\
                              & --  & 40.4 & 0.95 & 0.97 & 77.4 \\
\midrule
\multirow{2}{*}{ABC}          & 10k & 19.5 & 0.99 & 0.98 & 52.5 \\
                              & --  & 16.6 & 0.98 & 0.97 & 50.5 \\
\bottomrule
\end{tabular}
\caption{Generation statistical results across tokenization strategies. \textbf{MF}: measure-first; \textbf{PF}: part-first.}
\label{tab:generation_results}
\vspace{-1em}
\end{table}

==> tables/gpt_user_study.tex <==
\begin{table}[t]
\centering
\small
\begin{tabularx}{\columnwidth}{l l c c c c}
\toprule
\textbf{Tokenizer} & \textbf{BPE} & \textbf{Fid.} & \textbf{Corr.} & \textbf{Div.} & \textbf{Overall} \\
\midrule
\multirow{2}{*}{\libraryName\ MF} & --  & -- & -- & -- & -- \\
                            & 10k & -- & -- & -- & -- \\
\addlinespace
\multirow{2}{*}{\libraryName\ PF} & --  & -- & -- & -- & -- \\
                            & 10k & -- & -- & -- & -- \\
\addlinespace
\multirow{2}{*}{MIDI-REMI}    & --  & -- & -- & -- & -- \\
                            & 10k & -- & -- & -- & -- \\
\addlinespace
\multirow{2}{*}{ABC}     & --  & -- & -- & -- & -- \\
                            & 10k & -- & -- & -- & -- \\
\bottomrule
\end{tabularx}
\caption{Human pairwise-study results: Bradley--Terry scores with 95\% confidence intervals, per evaluation dimension. MF/PF = measure-first/part-first.}
\label{tab:user-study}
\end{table}
